Multi-Variate Time Series Forecasting on Variable Subsets

We formulate a new inference task in the domain of multivariate time series forecasting (MTSF), called Variable Subset Forecast (VSF), where only a small subset of the variables is available during inference. Variables are absent during inference because of long-term data loss (eg. sensor failures) or high -> low-resource domain shift between train / test. To the best of our knowledge, robustness of MTSF models in presence of such failures, has not been studied in the literature. Through extensive evaluation, we first show that the performance of state of the art methods degrade significantly in the VSF setting. We propose a non-parametric, wrapper technique that can be applied on top any existing forecast models. Through systematic experiments across 4 datasets and 5 forecast models, we show that our technique is able to recover close to 95\% performance of the models even when only 15\% of the original variables are present.

==> Arxiv Upload - MultiVariate Time Series Forecasting/intro.tex <==

\section{Introduction}
\label{sec:intro}
Multi-Variate Time Series Forecasting (MTSF) continues to receive significant attention from the research community owing to its applicability in many real-world scenarios\cite{han2021dynamic} 
such as traffic forecasting, air quality forecasting, power load forecasting and medical monitoring. We draw attention to two practical scenarios wherein MTSF models require robustness to data scarcity. Specifically, we present MTSF scenarios where at the time of  inference  the model does not have access to all the variables used in training. 

\noindent 
{\bf1. Long Term Variable Data Unavailability:}
In a majority of Multi-Variate Time Series applications, the most common source of  time series data is   via sensors. Each variable in the Multi-Variate Time Series is the output of a sensor. Sensor failures due to reasons like component malfunction, battery outages  are common in   real-world deployments where they are exposed to adverse weather conditions, dust  and so on. As explained in\cite{yick2008wireless} sensor failures can extend for a very long period of time (multiple months in many cases) before the sensor gets replaced. This causes long-term data unavailability for variables that were originally produced by the then-failed sensors. 

\begin{figure}[t]
	\centering
	%\includegraphics[scale=0.5]{images/Simple_Problem_Statement}
	\includegraphics[ width=75mm, height=45mm]{images/vsf_v9.jpg}
	
	\caption{Variable Subset Forecast Problem: The two sub-figures show a (i) training and (ii) test instance, respectively. The light gray part on top of each sub-figure represents the input timesteps. The dark shaded part is the forecast. %(where during training it incurs ground truth supervision loss).
	During training, Variables V1 through V7 are present while during Testing, only  V1, V2, V4, V7 are present.  } %Coloured nodes denote the presence of data whereas nodes filled white don't have any data. Associations are shown as a graph for intuitive understanding.	
	\label{fig:problem_statement}
\end{figure}


\noindent 
{\bf2. High$\rightarrow$Low Resource Domain Shift:}
Time Series models are  often used in domains that have a wide variability in resource availability. For instance,  consider  inventory prediction of products. This has been posed as a MTSF problem since there exists correlation in market demand across different products (for instance, phones and their cases~\cite{karb2020network}). A model trained on a dataset from large retailer will have a wide variety of products (variables). When applying the same model to a small and medium business(SMB) retailer, the number of products stocked will be significantly limited  and  may also vary over time. So it is not possible to  train a model on a fixed subset of products as the stocked items will vary across SMBs. 
%battery usage of apps in a low-spec smartphone, that does not have all the sensors than the high-end device that was used to generate the sensor data streams available during training\
Another example is a  MTSF model to forecast  physiological indicators like blood glucose, insulin, creatinine, etc\cite{cai2020time}. A model trained with data collected at a large hospital would have access to all the variables during training. When the same model is applied (at inference) in a rural hospital without access to many of the diagnostic instruments a large chunk of variables will be missing. In this case, though it is possible to know the subset of variables apriori, it is not scalable to create and maintain one model per known subset. Furthermore, the algorithm proposed in our work (section \ref{sec:our_method}) is able to outperform or match %perform upto 5\% better than 
a model that is trained on only a subset of the variables known apriori. Similar situations also occur in other domains such as   battery usage prediction between top-end  (high resource) and low-spec smartphones; and
%battery usage models trained on data from high-end phones (high resource) and applied on  low-spec smartphone data(low resource)\cite{kang2011personalized}, 
%inventory forecasting between large chain (high resource) and small-and-medium business(low resource) retailers\cite{karb2020network}
 wind speed forecasting between coastal (high resource) and deep-sea (low resource) naval stations\cite{hamid2018wind}. 

%wind speed using a variety of parameters like sea level pressure, dew point, rain intensity etc.  A remote station may not have all the 

%Sensor failure resilience is a key research topic in the sensor network community. 
Multi-Variate Time Series Imputation techniques\cite{luo2018multivariate, tang2020joint} are a relevant area of active research. Imputation methods use global inter-variable patterns  and local variable information  (average, recent values)   to generate plausible missing values. Imputation techniques significantly rely on temporal locality therefore are not very effective when the data is  missing for a  long time duration.  In the {\em High$\rightarrow$Low Resource Domain Shift} scenario, variables are missing entirely.  In this case, imputation methods are even less effective. 
%Because of these reasons, we argue that this scenario where variables are absent entirely during inference is different from the imputation problem statement.  
To the best of our knowledge, robustness of MTSF models in presence of such failures, that cause a subset of variables to be completely absent during inference, has not been studied in the literature. Although for completeness, we also provide a comparison to Imputation methods in section \ref{sec:comparison_imputation}.  




%The problem of MTSF aims to use past temporal data for multiple variables to predict the future values of the variables as accurately as possible. 
 


%With the shift of paradigm towards using machine learning to predict values for various events in future, the literature of time series forecasting has also seen a huge surge in the work done in the past few years. It has diverse implications in numerous real-world scenarios: forecasting speed of vehicles at intersections, predicting desired level of production for items in supply chains, predicting stock prices, predicting the electricity demands for various areas and various others. This can help people and entire corporations manage their decisions when the forecasts are accurate enough. 
%Given the past data for some variable, the problem of time series forecasting aims to predict the future values as accurately as possible. While univariate (single variable) time series forecasting is quite useful, the multivariate forecasting setup is much more interesting and seemingly relevant in practice. Unlike the univariate case 
Conventionally, the MTSF problem aims to simultaneously predict the future values of  $\mathcal{N}$ variables  given their past time series values by accurately modeling inter and intra variable dependencies.  In this paper,
%we propose a new inference task in the MTSF problem setup.  
the training setup is unchanged from the standard setting wherein we  assume 
%availability of  the entire dataset with
that the training algorithm has access to  all variables (denoted by $\mathcal{N}$). But during inference, the past data is only provided for an arbitrary small subset of variables (denoted by $\mathcal{S}$) and we aim to predict future values of variables in $\mathcal{S}$. We call this the {\em Variable Subset Forecast} (VSF in short) problem in MTSF. Figure \ref{fig:problem_statement} summarizes the problem with a simple example.  
% where $|\mathcal{S}| / |\mathcal{N}| \ll 1$.  

%The VSF problem, where only a random set of variables $(\mathcal{S})$ are only available during inference, can be seen in  two categories of real world scenarios: (i) {\em Intermittent Unavailability} due to  failure of multiple data producing nodes in the system (eg. sensors) (ii) {\em Domain Shift} where during inference we do not  permanently have all the variables used in training. 



%forecasting sales patterns of branded items in small markets (where a majority of sold items are non-branded) when the model was trained with data from larger markets (where most of the items sold are branded).
%In both the above scenarios the information available to the model during training is significantly different from what is available during inference. 
 
 The VSF problem  poses 2 key challenges. First, 
 %in order to make accurate predictions of the variables in $\mathcal{S}$ the forecast model might need access to variables beyond $\mathcal{S}$. 
 since a substantial portion of the data ($\mathcal{N-S}$ variables) 
 is absent during inference, it is challenging to recover the loss incurred compared to the setting where all $\mathcal{N}$ are present. 
  %.  
 Second, with only a small  $\mathcal{S}$ presented randomly during inference, it is not feasible to take advantage of the rich inter-variable associations in $\mathcal{N}$. Prior works \cite{wu2020connecting,Guo_Lin_Feng_Song_Wan_2019,10.1145/3209978.3210006,DBLP:journals/corr/abs-1803-01271} have shown significant performance gains by 
 exploiting such inter-variable dependencies.
 %is critical for improving performance on the MTSF task.  
 %we are not able make assumptions about the variable dependency graph structure during inference and hen
 Also, retraining the model for every subset $\mathcal{S}$ is not practically feasible since $\mathcal{S}$ is not known during training.
 
 In this paper, we also propose a novel solution to improve the performance of the forecasts models and show that it can even recover close to $95\%$ of the best-case performance even with only $15\%$ of the variables available. The proposed algorithm is a {\em wrapper method} in that it can be implemented over any existing forecast model. We take a non-parametric approach to addressing the problem by retrieving nearest neighbors using only the $\mathcal{S}$ variables and using these neighbors to fill missing values. However, this retrieval is inherently biased because neighbors are retrieved using a distance measure in partial dimensions and is therefore different from the traditional k-NN setting. Achieving near-optimal performance with a biased retrieval mechanism is another technical challenge we address. We propose a novel ensemble weighting method to score candidates from the biased retrieval. 
 %Interestingly, our algorithm can also recover close to actual performance of the forecast model even when only $15\%$ of the original set of variables $\mathcal{N}$ is available. 
 Our method is simple to implement and more importantly the underlying forecast models do not need re-training. 
 %which further supports our choice of using retrieval mechanism.  
 We make the following contributions in this paper:
 
 
 
 %and fast during runtime on any modern hardware.
 %In this paper we address two key challenges:   Working with  an unknown S and yet produce predictions close to an oracle setting  where data for all $\mathcal{N}$ variables are known.  


% Inspired by the recent success of non-parametric approaches for NMT also a very challenging problem.  


%We study the problem extensively from multiple angles in section \ref{sec:the_problem}. First, we verify the difficulty of this problem by showing that all the forecast models have a substantial increment in the error metrics used to quantify the performance. This is done by performing a comparison against the oracle case (where all data is available). Furthermore, we also show that even if the forecast models are trained with data of set $\mathcal{S}$ (which is infeasible in practice and only used for comparison), it can't outperform the oracle, thus the entire set $\mathcal{N}$ plays an important role in learning the underlying associations. A similar experiment along these lines is also performed to verify that removing the association learning modules significantly deteriorates the performance. We also verify that increasing the size of $\mathcal{S}$ leads to a monotonic decrease in the error metrics as a formal sanity check for this problem statement. Lastly, we note interesting patterns in the difference between error values of oracle and this subset prediction case with the variation in the forecast horizon length.


%A similar line of research underlying the idea of our algorithm has recently gained attention in NLP under the category of retrieval-based models which have shown nearly state of the art performance in many recent works tying multiple difficult NLP tasks. 
%We further provide extension of the algorithm to the popular ensemble technique and propose a non-trivial weight mechanism that has significant improvements over the standard averaging. To quantitatively and qualitatively understand the proposed algorithm as well as the datasets and models used, we perform thorough ablation studies and uncover some interesting properties detailed in section \ref{sec:our_method_empirical}. Lastly, we report an interesting finding in section \ref{subsec:pagerank_exps} which shows that the importance of a given set of variables correlates highly to increase in error metrics when the corresponding set of variables is removed, which can be used to develop sophisticated and more effective algorithms.

\begin{enumerate}
\item We formulate a new inference task called {\em Variable Subset Forecast} in MTSF motivated by  failure situations that arise in real-world settings. To the best of our knowledge we are the first to propose this problem formulation.  (Section~\ref{sec:the_problem}) 
 

\item We propose a novel {\em wrapper} solution to improve the performance of various models under this setup. The algorithm is very simple to code\footnote{Code available at  \href{https://github.com/google/vsf-time-series}{https://github.com/google/vsf-time-series}} and is agnostic to the choice of the forecast model. (Section~\ref{sec:our_method})

\item We conduct extensive experiments to understand why current forecast models significantly underperform in the VSF setting (Section~\ref{sec:performance_gap}). Then we quantitatively and qualitatively study our proposed solution with thorough ablations. %(Sections ~\ref{sec:empirical_evaluation}-\ref{sec:failure_analysis})

%have been performed to first show that this problem setup is non-trivial and leads to substantial increase in error metrics over standard forecasting where all variables are available.

\end{enumerate}




==> Arxiv Upload - MultiVariate Time Series Forecasting/related_work.tex <==
\section{Related Work}
%We first provide a brief survey of the different categories of methods proposed in time series forecasting literature followed by a quick history of the proposed problem statement.
%\subsection{Time series forecasting}
%  Models proposed for MTSF typically have two components: (i) first one learns the underlying associations amongst the variables (ii) the second one learns the temporal patterns for a given variables historical data. 
%These two components can further have complicated interpassed layers adhering to modern deep neural network practices. 
MTSF has a rich history with a diverse category of forecast methods proposed over decades. Some of the earliest models were based on \emph{Statistical Modelling}, which include: Vector Auto Regressive (VAR), Vector Auto Regressive Moving Average model (VARMA) \cite{Ltkepohl2005} as well as Gaussian Process (GP) based methods \cite{GP_time_series}. Another body of literature, although not extensive, is based on leveraging the Matrix Factorization (MF) techniques, which is detailed well in \cite{NIPS2016_85422afb}.
With the surge of Deep Neural models, there has been a series of architectural advances in this domain, which segregates the models into two typical components: (i) first one learns the underlying associations amongst the variables (referred as spatial module) (ii) the second one learns the temporal patterns for the variables' historical data (referred as temporal module). %These will be referred to as \emph{spatial} and \emph{temporal} modules/components in subsequent sections. 
%We elaborate these models in more detail as follows: 

%These models range from simple LSTM \cite{NIPS2014_a14ac55a, 10.1145/3097983.3098117} based models to deep convolutional networks (to learn variable associations) with recurrent mechanism (to model temporal patterns) \cite{10.1145/3209978.3210006, DBLP:journals/corr/abs-1809-04206}. More recently the graph based models have emerged as the state of the art\cite{ijcai2019-264, wu2020connecting, DBLP:journals/corr/abs-2007-02842, shang2021discrete} since they are able to model the variable inter-dependency better while still being expressive enough to model the temporal dimension of the problem.
 

%\textbf{Statistical Methods: } The earliest category of methods leverages statistical frameworks to forecast time series. Historical Averaging (HA) performs weighted linear combinations of the past data to predict the future values. Moving Average (MA), Auto Regressive (AR) and Auto Regressive Moving Average (ARMA) is another family of linear models with Autoregressive Integrated Moving Average (ARIMA) \cite{https://doi.org/10.1111/jtsa.12194} as a more advanced generalization. While these models handle univariate time series data, extensions of these methods such as Vector Auto Regressive (VAR) and Vector Auto Regressive Moving Average model (VARMA) \cite{Ltkepohl2005} have been proposed to capture the associations amongst the variables. From the Bayesian perspective, Gaussian Process (GP) based methods \cite{GP_time_series} have also been applied to model multivariate time series data. However, these methods are not scalable and make strong assumptions about the underlying data generating process.
%thus usually not performing well. 

%\textbf{Matrix Factorization Methods: } Another series of works in the literature, although not extensive, is based on leveraging the Matrix Factorization (MF) technique to learn low dimensional embeddings for the variables as well as the time steps. Most of these approaches utilize the framework of graph-based regularization in the temporal axis, with a graph explicitly encoding the temporal dependencies \cite{10.1007/978-3-540-45167-9_12}. In the work by \cite{conf/interspeech/WilsonRS08}, the authors use specially designed regularizers to encourage a log-normal structure on the temporal coefficients in the formulation. The work by \cite{NIPS2016_85422afb} proposed a temporal regularizer and generalized a series of prior works in the MF based time series forecasting research. Despite some improvements over the statistical approaches, these models can incur large runtime and require domain knowledge to carefully impose the temporal regularization. 

% \textbf{Deep Learning Based Methods: } %While the non-deep learning categories of methods have multiple caveats, 
% Deep learning techniques that are from various assumptions of statistical models and scalable have become state of the art across almost all benchmarks. For handling univariate time series, %the popular family of Long Short Term Memory (LSTMs) 
% LSTMs were applied in some of the primary works \cite{NIPS2014_a14ac55a}, followed by other works such as DeepAR \cite{salinas2020deepar}.% that perform accurate probabilistic forecasts based on training a recurrent network model. %More advanced models such as SMF \cite{10.1145/3097983.3098117} and N-BEATS \cite{Oreshkin2020N-BEATS} (consisting of backward and forward residual links as well as MLPs ) were then proposed that leverage much deeper architectures and modern tweaks. 
% To generalize to the multivariate forecast setting (all $\mathcal{N}$ variables forecasted together), \cite{10.1145/3209978.3210006, DBLP:journals/corr/abs-1809-04206}%, DBLP:journals/corr/abs-1803-01271} 
% proposed some of the first models. %The high level architecture of both these works follow a similar pattern. A recurrent neural network (RNN) is applied on the temporal axis to model the time variation and a convolutional neural network (CNN) is applied to capture the interaction amongst multiple variables. 
% Other sophisticated models include DeepState \cite{NEURIPS2018_5cf68969} that combines state space models with deep recurrent neural networks. %Transformers \cite{NIPS2017_3f5ee243} have shown state of the art performance on a diverse set of tasks and recently leveraged for time series forecasting problem \cite{DBLP:journals/corr/abs-2001-08317} with its generalization to the multivariate settings by \cite{10.1145/3447548.3467401, DBLP:journals/corr/abs-2109-12218}. However, unlike graph-based models (defined next), it is non-trivial for the transformer architecture to incorporate the scenario where each variable can have an embedding with dimension more than one (ie a vector instead of a scalar  value) at each time step and will require extension to higher order attention mechanism \cite{DBLP:journals/corr/abs-2110-14416}. This can happen in the cases where auxiliary information is used. 
% Transformers \cite{NIPS2017_3f5ee243} have shown state of the art performance on a diverse set of tasks and recently leveraged for time series forecasting problem \cite{10.1145/3447548.3467401}. %However, unlike graph-based models (defined next), it is non-trivial for the transformer architecture to incorporate the scenario where each variable can have an embedding with dimension more than one (ie a vector instead of a scalar  value) at each time step and will require extension to higher order attention mechanism. This can happen in the cases where auxiliary information is used. 
% A huge bottleneck of these works is that interaction amongst the variables is encapsulated in a global hidden vector which fails to explicitly model the pairwise dependencies and interactions. 

% \textbf{Graph Based Deep Learning Methods: } More recently, graph neural network (GNN) based approaches have been shown to work well to model various types of spatio-temporal data spanning across tasks such as regression, classification, clustering etc. %The literature of GNNs has a vast categorization of proposed methods including graph convolution \cite{DBLP:journals/corr/KipfW16}, graph attention \cite{veli_2018graph}, higher order \cite{pmlr-v97-abu-el-haija19a} and various others. 
% The success of GNN based methods is attributed to the fact they can explicitly model the dependencies amongst the pairs of nodes (or variables) in the graph and iteratively update the representations by aggregating information. %from neighbors of a given node (this is more commonly referred to as the message passing framework of GNNs). 
% In the spatio-temporal setting, the temporal dependencies are usually modelled by RNN whereas a GNN is applied on the spatial axis with a predefined input graph. This general framework was initially proposed in traffic prediction models such as DCRNN \cite{li2018diffusion}%, STGCN \cite{ijcai2018-505} 
% as well as for skeleton-based action recognition \cite{Yan_Xiong_Lin_2018} %\cite{Yan_Xiong_Lin_2018, DBLP:journals/corr/abs-1805-07694} 
% but was later adopted for multivariate time series forecasting as well \cite{Guo_Lin_Feng_Song_Wan_2019}. In some cases, where the time series forecasting problem doesn't have a predefined graph, which also synonymously represents the associations amongst variables, approaches such as \cite{wu2020connecting, ijcai2019-264} have been proposed which explicitly learn the graph structure as part of the optimization procedure. Also, interestingly some of these approaches such as \cite{ijcai2019-264, wu2020connecting} etc employ a temporal convolution layer \cite{DBLP:journals/corr/LeaFVRH16} 
% instead of RNNs which make the runtime substantially faster with its performance being on par with the former. 

%We thus select $5$ widely used forecast models consisting of $3$ Graph based: MTGNN \cite{wu2020connecting}, ASTGCN \cite{Guo_Lin_Feng_Song_Wan_2019}, MSTGCN \cite{Guo_Lin_Feng_Song_Wan_2019} and $2$ Deep Learning based: LSTNet \cite{10.1145/3209978.3210006}, TCN \cite{DBLP:journals/corr/abs-1803-01271}.

The popular works of \cite{10.1145/3209978.3210006, DBLP:journals/corr/abs-1809-04206} provided some of the first LSTM based multivariate forecasting models, followed by more sophisticated models such as DeepState \cite{NEURIPS2018_5cf68969} and subsequently Transformers \cite{10.1145/3447548.3467401}. A huge bottleneck of these works is that interaction amongst the variables is encapsulated in a global hidden vector which fails to explicitly model the pairwise dependencies and interactions. To tackle this, GNN-based models have become the SOTA in recent years. Here, the temporal dependencies are usually modelled by RNN whereas a GNN is applied on the spatial axis. This general framework was initially proposed in traffic prediction models such as DCRNN \cite{li2018diffusion} as well as for skeleton-based action recognition \cite{Yan_Xiong_Lin_2018} but was later adopted for multivariate time series forecasting as well \cite{Guo_Lin_Feng_Song_Wan_2019}. 

  
For our experiments,  we select the following $5$ widely used forecast models 
as a representation of the wide variety of recent techniques in literature -  \textbf{(i) MTGNN} \cite{wu2020connecting}:  This method extracts uni-directed relations among the time series variables via a graph learning module and then performs spatio-temporal modelling, where the temporal module is a temporal convolution network. \textbf{(ii) ASTGCN} \cite{Guo_Lin_Feng_Song_Wan_2019}: This method utilizes a spatial-temporal attention mechanism to learn the dynamic spatial and temporal correlations of the data and then leverages a standard spatio-temporal modelling mechanism for forecasting. \textbf{(iii) MSTGCN} \cite{Guo_Lin_Feng_Song_Wan_2019}: This method utilizes graph convolutional networks for capturing the spatial features and convolutions in the temporal dimension for describing dependencies from nearby time slices, to learn to forecast. \textbf{(iv) LSTNet} \cite{10.1145/3209978.3210006}: This model uses convolutions on the spatial axis to discover the associations amongst the variables while a recurrent network is applied on the temporal axis. \textbf{(v) TCN} \cite{DBLP:journals/corr/abs-1803-01271}: This is a completely convolutional neural network based model that combines various practices such as residual connections and dilations with causal convolutions and perform predictions autoregressively.

%of $3$ Graph based and $2$ Deep Learning based models as follows.   
 %consider some of the recent state of the art multivariate time series forecasting models which have shown reasonably good results across multiple benchmarks. A brief and high level detail for each model is described below:
%  \begin{itemize}
%      \item {MTGNN \cite{wu2020connecting}: } This method extracts uni-directed relations among the time series variables via a graph learning module and then performs spatio-temporal modelling, where the temporal module is a temporal convolution network.
%      %\item {GWNET (Graph Wave Net) \cite{ijcai2019-264}: } This method first learns the underlying associations among the time series variables with a learnable adjacency matrix module and then applies spatio-temporal modelling with a gating mechanism as well.
%      \item {ASTGCN \cite{Guo_Lin_Feng_Song_Wan_2019}: } This method utilizes a spatial-temporal attention mechanism to learn the dynamic spatial and temporal correlations of the data and then leverages a standard spatio-temporal modelling mechanism for forecasting.  
%      \item {MSTGCN \cite{Guo_Lin_Feng_Song_Wan_2019}: } This method utilizes graph convolutional networks for capturing the spatial features and convolutions in the temporal dimension for describing dependencies from nearby time slices, to learn to forecast.
%      \item {LSTNet \cite{10.1145/3209978.3210006}: } This model uses convolutions on the spatial axis to discover the associations amongst the variables while a recurrent network is applied on the temporal axis.
%     \item {TCN \cite{DBLP:journals/corr/abs-1803-01271}: } This is a completely convolutional neural network based model that combines various practices such as residual connections and dilations with causal convolutions and perform predictions autoregressively.
%  \end{itemize}



==> Arxiv Upload - MultiVariate Time Series Forecasting/scalable_part.tex <==
\section{Scalable k-NN Heuristics for VSF}
Fast Nearest Neighbor Search that scales to billions of datapoints is a topic of active research\cite{johnson2019billion}. For the techniques proposed in this paper, a variation of k-NN retrieval is needed where the similarity needs to be computed on a subset of dimensions.
An optimal solution to this problem is an open research problem by itself and is hence out of scope for this paper. In this section, we present a practical implementation that scales and performs  well.% for the datasets used in this paper. 

\subsection{Pre-Processing}
%\textbf{Pre-Processing:} 
Let $P$ be the forecast time steps that we assume is known during the database construction time and $|\mathcal{T}|$ be the total number of training records (or instances), where each record is a tensor of shape $P \times |\mathcal{N}|$. For ease of notation, we consider $D=1$, however the methodolgy follows for any $D>1$ as well. %We denote $R_i$ to be tbe $i^{th}$ record in the training data, a vector of dimension $N$ which is the number of variables. 
We construct a new table, henceforth called the {\em Query Table} in which each row contains an instance of $\mathcal{T}$, flattened into a vector of shape $P * |\mathcal{N}|$. %$P$ consecutive instances of training data in the original table are flattened into one row into the Query Table. A moving window of size $P$ is advanced by one to created the next row of the Query Table. Hence the original table will have $T$ rows with $|\mathcal{N}|$  columns while the {\em Query Table} 
Therefore, the {\em Query Table} will have $|\mathcal{T}|$ rows and $P * |\mathcal{N}|$ columns. Since all the columns are continuous real valued numbers, we   create indexes that are efficient for range queries. 


%which contains all the instances in the training data in the flattened for(defined previously in section \ref{subsec:borrowing_data}), thus having $P * |\mathcal{N}| * D$ columns . %We use a moving window of height $P$ on the input table and flatten all the records inside the moving window to create a corresponding record. Specifically if the moving window is between the first record and the $M^{th}$ record, we create the first record of the new table as the $M$ records in the original table placed horizontally. The new table hence will have $M . N$ columns For each of the  $N$ variables in a given dataset we calculate the mean $\mu_i$ standard deviation $\sigma_i$ for every variable.  


\subsection{Methodology}
%\textbf{Methodology:} 
Our task remains the same as defined in section \ref{subsec:borrowing_data}: to retrieve $m$ neighbors for the test instance $X^{test}$. We do this by performing  query on the Query Table that has  $F = P * |\mathcal{S}| $ sub-queries. Each sub-query is a range query on a {\em Query Table} column.   For each sub-query $X^{test}_{[p,s]}$ of the tensor $X^{test}$, we find the instance $X^{prime}$ in the {\em Query Table} satisfying the following:
\begin{equation}
    \label{eq:db_search}
    |X^{test}_{[p,s]} - X^{prime}_{[p*|\mathcal{N}| + \sigma(s)]}| \leq b_{\sigma(s)}
\end{equation}
where $\sigma(s)$ is the projection of $s$ to its actual variable in $\mathcal{S}$, $b_{\sigma(s)}$ is a hyperparameter for the corresponding variable. $X^{prime}$ is used as a vector in above equation (note the shape of $X^{prime}$ is $P * |\mathcal{N}|$) with the corresponding element vector indexed by $[p*|\mathcal{N}| + \sigma(s)]$. The set of indices in the table for all such $X^{prime}$ is denoted by $\mathcal{I}({p,s})$. 

Lastly, we obtain the set of desired neighbors by performing intersection of the sets for all elements of $X^{test}$, given by $\mathcal{I} = \bigcap\limits_{p=1}^{P}\bigcap\limits_{s=1}^{|\mathcal{S}|}\mathcal{I}({p,s})$. 

This operation is repeated until we obtain the desired number of $m$ neighbors, thus incurring $\geq 1$ rounds with expansion of $\mathcal{I}$ in each round. In each subsequent round, we multiply some of the $b_{\sigma(s)}$ (out of the total $|\mathcal{S}|$) for which the \emph{L.H.S} of equation \ref{eq:db_search} is tighest w.r.t to $b_{\sigma(s)}$ by a constant factor $u > 1$, which implies loosening the constraints to obtain a larger set.
Since, $|\mathcal{I}| \geq m$, we also perform a linear search over the retrieved neighbors, indexed via $\mathcal{I}$, and retrieve the top-$m$.

\textbf{Selection of Primary Values of $b_{\sigma(s)}$:} We treat $b_{\sigma(s)}$ as hyperparameter for this experiment. Since searching for the value of $b_{\sigma(s)}$ over the real line is difficult, we utilize the training and validation set as follows: (i) for each instance in the validation set, obtain its $\hat{k}^{th}$ neighbor ($\hat{k}$ is a hyperparameter) by using all $\mathcal{N}$ variables, (ii) compute the average distance, w.r.t to the variable dimension, over the $\hat{k}^{th}$ neighbors for all the val set instances. This provides a reasonable proxy to issue a query and perform the search in equation \ref{eq:db_search} for the corresponding $b_{\sigma(s)}$.% of any variable in $\mathcal{S}$.


\subsection{Experimental Results}

\textbf{Query-Time:}
%During query time, we need to find k nearest neighbors for a given point $V$ of $S$ variables and $M$ time steps. Since the Query Table indexes all the time steps, we create range query with $S*M$ conjunctions. The range for a given variable is given as $\mu_i - \sigma_i \leq$  $V_i$ $\leq \mu_i + \sigma_i$. Since we use range queries on dense columns, query plans on standard databases are able to optimize this type of query well based on pre-constructed histograms. A sample query plan is shown in Appendix\ref{sec:query_plan}  If we are able to retrieve $k$ neighbors in a round, the round ends there. Else we need to relax the conjunctions to retrieve more neighbors. In order to choose the conjunction to relax, we pick top-$l$ conjunctions by the distance of the  closest retrieved neighbor to the boundary. For the relaxed conjunctions we exponentially double the range; so for the second round it would be  $\mu_i - 2*\sigma_i \leq$  $V_i$ $\leq \mu_i + 2*\sigma_i$ and for the 3rd round  $\mu_i - 4*\sigma_i \leq$  $V_i$ $\leq \mu_i + 4*\sigma_i$ and so on.  We set $l \eq 5$ in our experiments.   
Figure \ref{fig:scalability_figs} shows the number of rounds required to fetch desired number of neighbors, averaged over $100$ selections of $\mathcal{S}$. As we can see for most of the neighborhood settings experimented in section \ref{subsec:vary_num_neighbors}, we are able retrieve neighbors in at most 3 rounds, with a diminishing increase. The total time incurred is the sum of database search and a linear search over the training instances corresponding to indices in $\mathcal{I}$ (which is a small set), both of which are very fast operations. \\ %A more systematic and scalable solution to this problem is delegated to future work. 


\begin{figure}[h]
    \centering
	\includegraphics[width=\linewidth]{images/scalability/all_figure}
	
	\caption{Variation of the average number of rounds taken against the desired number of neighbors to fetch. Experimented for MTGNN on ECG5000.}	
	\label{fig:scalability_figs}
\end{figure}

% \begin{wrapfigure}{R}{0.25\textwidth}
% % \begin{figure}[h]
%     % \centering
% 	\includegraphics[width=0.25\textwidth]{images/scalability/all_figure}
	
% 	\caption{Average number of rounds against the desired number of neighbors to fetch.}	
% 	\label{fig:scalability_figs}
% % \end{figure}
% \end{wrapfigure}



\textbf{Performance Comparison to Direct Neighbor Retrieval (Section \ref{sec:empirical_evaluation}):} We provide a comparison for the values of $\Delta_{Ensemble}$ in the two settings where we retrieve the desired $m$ neighbors via: (i) \emph{Direct} Retrieval (from table \ref{table:ewp_main}) to the neighbors obtained using the approach in this section referred as \emph{Scalable} Retrieval. From the results provided in table \ref{table:scalability_ewp_delta}, its evident that the proposed \emph{scalable search} approach retrieves reasonably good neighbors and can recover performance very close to the \emph{Direct} retrieval. We explicitly call out that the hyperparameters: $b_{\sigma(s)}$, size of $\mathcal{I}$ and the constant multiplication factor $u$ , directly governs the results and thus require careful tuning to provide the desired level of runtime-performance tradeoff.

\begin{table}[h]
\small

\caption{Comparison of $\Delta_{Ensemble}$ for neighbor retrieval using: (i) \emph{Direct} (from table \ref{table:ewp_main}) vs (ii) \emph{Scalable} (proposed in this section) for MTGNN model} 
\label{table:scalability_ewp_delta}

\centering
\setlength\tabcolsep{3.5pt}
\begin{tabular}{|l|rr|rr|}

\hline
   &  \multicolumn{2}{c|}{\bf \emph{SOLAR}}  &  \multicolumn{2}{c|}{\bf \emph{ECG5000}}  \\
\cline{1-5}  
Retrieval &  MAE  & RMSE & MAE & RMSE \\ 
\hline

% \multicolumn{5}{c}{\bf \emph{Main Results}} \\
\hline
\emph{$\Delta_{Ensemble}$ \emph{Direct}} & 30.05 \% & 25.45 \% & 2.14 \% & 3.11 \% \\
\emph{$\Delta_{Ensemble}$ \emph{Scalable}} & 31.28 \% & 26.83 \% & 2.51 \% & 3.29 \% \\
\hline 

\end{tabular}

\end{table}

